Object Rearrangement with Nested Nonprehensile Manipulation Actions

This paper considers the problem of rearrangement planning, i.e finding a sequence of manipulation actions that displace multiple objects from an initial configuration to a given goal configuration. Rearrangement is a critical skill for robots so that they can effectively operate in confined spaces that contain clutter. Examples of tasks that require rearrangement include packing objects inside a bin, wherein objects need to lay according to a predefined pattern. In tight bins, collision-free grasps are often unavailable. Nonprehensile actions, such as pushing and sliding, are preferred because they can be performed using minimalistic end-effectors that can easily be inserted in the bin. Rearrangement with nonprehensile actions is a challenging problem as it requires reasoning about object interactions in a combinatorially large configuration space of multiple objects. This work revisits several existing rearrangement planning techniques and introduces a new one that exploits nested nonprehensile actions by pushing several similar objects simultaneously along the same path, which removes the need to rearrange each object individually. Experiments in simulation and using a real Kuka robotic arm show the ability of the proposed approach to solve difficult rearrangement tasks while reducing the length of the end-effector's trajectories.

==> baselines.tex <==
We present here three generic methods that are related to the proposed approach and that will be used for comparisons. 

%\subsection{Collision-free Individual Planning}

\subsection{Monotone Rearrangement Search (MRS)}
The MRS algorithm is given in Algorithm~\ref{alg:mrs} and is an adaptation of an existing rearrangement planning algorithm~\cite{Krontiris-RSS-15}, which itself is an adaptation of a NAMO approach for clearing paths to unreachable objects~\cite{Stilman2007ManipulationPA}. The original algorithm of ~\cite{Stilman2007ManipulationPA} is limited to . 
\begin{algorithm}[h]
\KwIn{workspace $\mathcal{W}$, objects $O$, spatial window $w$, object configurations $c$, goal arrangement $c_{goal}$, radius $r$}
\KwOut{a sequence of actions $\pi$}
$G_\mathcal{W} \leftarrow \text{Roadmap}(\mathcal{W})$\\
\ForEach{ $c^i \in c, c^i_{goal} \in c_{goal}$ }
{
    \If{ $|c^i - c^i_{goal}| > \epsilon$ }
    {
        $v^i_{0} \leftarrow \text{GetLocation}(c^i)$\\
        $v^i_{1} \leftarrow \text{GetLocation}(c^i_{goal})$\\
        add $v_0^i, v_1^i$ to $G_\mathcal{W}$ and connect to the nearest\\
        $(\pi',c) \leftarrow \text{SlideWindow}(G_{\mathcal{W}},w,v^i_{0},v^i_{1},c,\{o^i\},r)$\\
        $\pi.\text{PushBack}(\pi')$\\
        move $w$ centered on $v^i_{1}$\\
        $(\pi'',c) \leftarrow \text{KinodynamicRRT}(w,c,c_{goal},\{o^i\},\mathcal{W})$\\
        $\pi.\text{PushBack}(\pi'')$
    }
}
\caption{Monotone Rearrangement Search (MRS)}
\label{alg:mrs}
\end{algorithm}

\subsection{Collision-free Joint Planning}
Barry2012
Jentzsch2015

\subsection{Kinodynamic Planning}


